Higher geometry for non-geometric T-duals

We investigate topological T-duality in the framework of non-abelian gerbes and higher gauge groups. We show that this framework admits the gluing of locally defined T-duals, in situations where no globally defined ("geometric") T-duals exists. The gluing results into new, higher-geometrical objects that can be used to study non-geometric T-duals, alternatively to other approaches like non-commutative geometry.

==> kobib.tex <==
\makeatletter

\def\kobiburl#1{
   \IfSubStr
     {#1}
     {://arxiv.org/abs/}
     {\kobibarxiv{#1}}
     {\kobiblink{#1}}}
\def\kobibarxiv#1{\href{#1}{\texttt{[arxiv:\StrGobbleLeft{#1}{21}]}}}
\def\kobiblink#1{
  \StrSubstitute{#1}{\~{}}{\string~}[\myurl]
  \StrSubstitute{#1}{_}{\underline{\;\;}}[\mylink]
  \StrSubstitute{\mylink}{&}{\&}[\mylink]
  \StrSubstitute{\mylink}{/}{/\allowbreak}[\mylink]
  \newline Available as: \mbox{\;}
  \href{\myurl}{\texttt{\mylink}}}

\def\noarxiv{\def\kobibarxiv##1{}}
\def\nolinks{\def\kobiblink##1{}}

\renewenvironment{thebibliography}[1]
     {\ifx\relax#1\relax\else
      \if!\refname!\else
        \tocsection{\refname}
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}%
      \fi
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m
      \fi}

\makeatother




==> theorems.tex <==
\makeatletter

\def\theoremsintoc{\addtotheorempostheadhook{
  \ifnum\c@secnumdepth=0\addcontentsline{toc}{section}{\@currenvir\space\@currentlabel}\fi
  \ifnum\c@secnumdepth=1\addcontentsline{toc}{subsection}{\@currenvir\space\@currentlabel}\fi
  \ifnum\c@secnumdepth=2\addcontentsline{toc}{subsubsection}{\@currenvir\space\@currentlabel}\fi
  \ifnum\c@secnumdepth=3\addcontentsline{toc}{subsubsubsection}{\@currenvir\space\@currentlabel}\fi
}}


\def\setsecnumdepth#1{
  \setcounter{secnumdepth}{#1}
  \setcounter{equation}{0}
  \setcounter{theorem}{0}
  \ifnum\c@secnumdepth=0
    \counterwithout{equation}{section}
    \counterwithout{equation}{subsection}
    \counterwithout{equation}{subsubsection}
    \def\thetheorem{\arabic{theorem}}    
    \def\theproposition{\arabic{proposition}}    
    \def\thecorollary{\arabic{corollary}}    
    \def\thedefinition{\arabic{definition}}    
    \def\theconstruction{\arabic{construction}}    
    \def\thelemma{\arabic{lemma}}    
    \def\theremark{\arabic{remark}}    
    \def\theproblem{\arabic{problem}}    
    \def\theexample{\arabic{example}}    
    \def\thefigure{\arabic{figure}}    
    \def\theexercise{\arabic{exercise}}    
  \fi
  \ifnum\c@secnumdepth=1
    \counterwithin{equation}{section}
    \counterwithin{theorem}{section}
    \def\theequation{\thesection.\arabic{equation}}    
    \def\thetheorem{\thesection.\arabic{theorem}}    
    \def\theproposition{\thesection.\arabic{proposition}}    
    \def\thecorollary{\thesection.\arabic{corollary}}    
    \def\thedefinition{\thesection.\arabic{definition}}    
    \def\theconstruction{\thesection.\arabic{construction}}    
    \def\thelemma{\thesection.\arabic{lemma}}    
    \def\theremark{\thesection.\arabic{remark}}    
    \def\theproblem{\thesection.\arabic{problem}}    
    \def\theexample{\thesection.\arabic{example}}    
    \def\thefigure{\thesection.\arabic{figure}}    
    \def\theexercise{\thesection.\arabic{exercise}}    
  \fi
  \ifnum\c@secnumdepth=2
    \counterwithin{equation}{subsection}
    \counterwithin{theorem}{subsection}
    \def\theequation{\thesubsection.\arabic{equation}}    
    \def\thetheorem{\thesubsection.\arabic{theorem}}    
    \def\theproposition{\thesubsection.\arabic{proposition}}    
    \def\thecorollary{\thesubsection.\arabic{corollary}}    
    \def\thedefinition{\thesubsection.\arabic{definition}}    
    \def\theconstruction{\thesubsection.\arabic{construction}}    
    \def\thelemma{\thesubsection.\arabic{lemma}}    
    \def\theremark{\thesubsection.\arabic{remark}}    
    \def\theproblem{\thesubsection.\arabic{problem}}    
    \def\theexample{\thesubsection.\arabic{example}}    
    \def\thefigure{\thesubsection.\arabic{figure}}    
    \def\theexercise{\thesubsection.\arabic{exercise}}    
  \fi  
  \ifnum\c@secnumdepth>2
    \counterwithin{equation}{subsubsection}
    \counterwithin{theorem}{subsubsection}
    \def\theequation{\thesubsubsection.\arabic{equation}}    
    \def\thetheorem{\thesubsubsection.\arabic{theorem}}    
    \def\theproposition{\thesubsubsection.\arabic{proposition}}    
    \def\thecorollary{\thesubsubsection.\arabic{corollary}}    
    \def\thedefinition{\thesubsubsection.\arabic{definition}}    
    \def\theconstruction{\thesubsubsection.\arabic{construction}}    
    \def\thelemma{\thesubsubsection.\arabic{lemma}}    
    \def\theremark{\thesubsubsection.\arabic{remark}}    
    \def\theproblem{\thesubsubsection.\arabic{problem}}    
    \def\theexample{\thesubsubsection.\arabic{example}}    
    \def\thefigure{\thesubsubsection.\arabic{figure}}    
    \def\theexercise{\thesubsubsection.\arabic{exercise}}    
  \fi  
}

%%% Theoreme definieren

\newlength{\theoremspace}
\setlength{\theoremspace}{1em}

\def\@theoremheadend{.}

\newtheoremstyle{theorem}          {\theoremspace}{\theoremspace}{\normalfont\itshape}{0pt}{\normalfont\bfseries}{\@theoremheadend}{ }{\thmname{#1}\space\thmnumber{#2}\thmnote{ (#3)}}
\newtheoremstyle{corollaryof}      {\theoremspace}{\theoremspace}{\normalfont\itshape}{0pt}{\normalfont\bfseries}{\@theoremheadend}{ }{\thmname{#1}\space\thmnumber{#2}\thmnote{ aus #3}}
\newtheoremstyle{remark}           {\theoremspace}{\theoremspace}{\normalfont}        {0pt}{\normalfont\itshape} {\@theoremheadend}{ }{\thmname{#1}\space\thmnumber{#2}\thmnote{ (#3)}}
\newtheoremstyle{remarkunnumbered} {\theoremspace}{\theoremspace}{\normalfont}        {0pt}{\normalfont\itshape} {\@theoremheadend}{ }{\thmname{#1}}

\declaretheorem[style=theorem,numberwithin=subsubsection,name=\nameTheorem]{theorem}
\declaretheorem[style=theorem,name=\nameProposition,sibling=theorem]{proposition}
\declaretheorem[style=theorem,name=\nameDefinition,sibling=theorem]{definition}
\declaretheorem[style=theorem,name=\nameLemma,sibling=theorem]{lemma}
\declaretheorem[style=theorem,name=\nameCorollary,sibling=theorem]{corollary}


\declaretheorem[style=theorem,name=\nameTheorem]{maintheorem}
\declaretheorem[style=theorem,name=\nameProposition,sibling=maintheorem]{mainproposition}
\declaretheorem[style=theorem,name=\nameCorollary,sibling=maintheorem]{maincorollary}
\declaretheorem[style=theorem,name=\nameDefinition,sibling=maintheorem]{maindefinition}

\declaretheorem[style=remark,name=\nameRemark,sibling=theorem]{remark}
\declaretheorem[style=remark,name=\nameConstruction,sibling=theorem]{construction}
\declaretheorem[style=remark,name=\nameProblem,sibling=theorem]{problem}
\declaretheorem[style=remark,name=\nameExample,sibling=theorem]{example}
\declaretheorem[style=remark,name=\nameExercise,sibling=theorem]{exercise}
\declaretheorem[style=remarkunnumbered,name=\nameExample,numbered=no]{example*}
\declaretheorem[style=remarkunnumbered,name=\nameRemark,numbered=no]{remark*}

%% corollaryofbody wird nur als Vorstufe von corollaryof definiert.
\declaretheorem[style=corollaryof,name=\nameCorollary]{corollaryofbody}


%%% Cref konfiguieren

\def\setcrefnames{
  \crefname{theorem}{\nameTheorem}{\nameTheorems}
  \Crefname{theorem}{\nameTheorem}{\nameTheorems}
  \crefname{maintheorem}{\nameTheorem}{\nameTheorems}
  \Crefname{maintheorem}{\nameTheorem}{\nameTheorems}
  \crefname{definition}{\nameDefinition}{\nameDefinitions}
  \Crefname{definition}{\nameDefinition}{\nameDefinitions}
  \crefname{construction}{\nameConstruction}{\nameConstructions}
  \Crefname{construction}{\nameConstruction}{\nameConstructions}
  \crefname{corollary}{\nameCorollary}{\nameCorollaries}
  \Crefname{corollary}{\nameCorollary}{\nameCorollaries}
  \crefname{corollaryofbody}{\nameCorollary}{\nameCorollaries}
  \Crefname{corollaryofbody}{\nameCorollary}{\nameCorollaries}
  \crefname{proposition}{\nameProposition}{\namePropositions}
  \Crefname{proposition}{\nameProposition}{\namePropositions}
  \crefname{lemma}{\nameLemma}{\nameLemmas}
  \Crefname{lemma}{\nameLemma}{\nameLemmas}
  \crefname{remark}{\nameRemark}{\nameRemarks}
  \Crefname{remark}{\nameRemark}{\nameRemarks}
  \crefname{remark*}{\nameRemark}{\nameRemarks}
  \Crefname{remark*}{\nameRemark}{\nameRemarks}
  \crefname{problem}{\nameProblem}{\nameProblems}
  \Crefname{problem}{\nameProblem}{\nameProblems}
  \crefname{example}{\nameExample}{\nameExamples}
  \Crefname{example}{\nameExample}{\nameExamples}
  \crefname{example*}{\nameExample}{\nameExamples}
  \Crefname{example*}{\nameExample}{\nameExamples}
  \crefname{exercise}{\nameExercise}{\nameExercises}
  \Crefname{exercise}{\nameExercise}{\nameExercises}
  \crefname{section}{\nameSection}{\nameSections}
  \Crefname{section}{\nameSection}{\nameSections}
  \crefname{appendix}{\nameAppendix}{\nameAppendixs}
  \Crefname{appendix}{\nameAppendix}{\nameAppendixs}
  \crefname{figure}{\nameFigure}{\nameFigures}
  \Crefname{figure}{\nameFigure}{\nameFigures}
  \crefname{enumi}{\unskip}{\unskip}
  \Crefname{enumi}{\unskip}{\unskip}
  \crefname{equation}{\nameEquation}{\nameEquations}
  \Crefname{equation}{\nameEquation}{\nameEquations}
  \crefname{}{\unskip}{\unskip}
  \Crefname{}{\unskip}{\unskip}
}

\setcrefnames
%\crefformat{}{#2#1#3}

%%% Parentlabel belegen

\def\@parenttype{}
\def\@parentcounter{}

\addtotheorempostheadhook{%
  \protected@edef\@parenttype{\@currenvir}%
  \protected@edef\@parentcounter{\@currentlabel}%
  \def\@tempa{theorem}
  \ifx\@currenvir\@tempa\setcounter{corollaryofbody}{0}\else\relax\fi%
}

%%% Liste nur in neuer Zeile beginnen

\addtotheorempostheadhook{\leavevmode}

%%%% Verweise auf Enumerate %%%%

\def\clabel#1{%
  % Label für Bakoma \cref{*}
  \protected@edef\@currentlabel{\csname label\@enumctr\endcsname}%
  \cref@old@label{#1*}% 
  %
  % Label für Bakoma \cref{}
  \protected@edef\@currentlabel{\@parentcounter\space\csname label\@enumctr\endcsname}%
  \cref@old@label{#1}
  %
  % Label für MikTeX \cref{*}
  \protected@edef\@currentlabel{[enumi][\arabic{enumi}][]\csname label\@enumctr\endcsname}%
  \@bsphack
  \protected@write\@auxout{}%
         {\string\newlabel{#1*@cref}{{\@currentlabel}{\thepage}}}%
  \@esphack
  %  
  % Label für MikTeX \cref{}
  \protected@edef\@currentlabel{[\@parenttype][\arabic{enumi}][]\@parentcounter\space\csname label\@enumctr\endcsname}%
  \@bsphack
  \protected@write\@auxout{}%
         {\string\newlabel{#1@cref}{{\@currentlabel}{\thepage}}}%
  \@esphack
  }

\AtBeginDocument{%
  \let\@oldlabel\label%
  \def\label#1{\def\@tempa{enumerate}\ifx\@tempa\@currenvir\clabel{#1}\else\@oldlabel{#1}\fi}}


%%% \ctype gibt den Typ eines Labels zurück, also z.B. "Satz", wenn #1 auf einen Satz zeigt.

\def\ctype#1{%
  \def\@namecref@labelexists{0}%
  \expandafter\ifx\csname r@#1@cref\endcsname\relax%
    %%% Es gibt keinen Miktex-Label
  \else%
    \def\@namecref@labelexists{1}%
  \fi%
  \expandafter\ifx\csname r@#1\endcsname\relax%
    %%% Es gibt keinen Bakoma-Label
  \else%
    \def\@namecref@labelexists{1}%
  \fi%
  \ifnum\@namecref@labelexists=0%
    \protect\G@refundefinedtrue%
    \nfss@text{\reset@font\bfseries ??}%
    \@latex@warning{Reference `#1' on page \thepage \space undefined}%
  \else%
    \cref@gettype{#1}{\@tempa}%
    \expandafter\csname cref@\@tempa @name\endcsname%
  \fi%
}

%%% \nameref gibt den Namen eines Labels zurück, der z.B. mit begin{theorem}[Name] eingerichtet wurde

%%% \namecref gibt die Normale Nummer sowie - falls vorhanden - den Namen in Anführungszeichen zurück


%
% Das hier sollte nur aufgerufen werden, wenn die Existenz des Labels geprüft wurde
%
\def\@namecref#1{%
    \cref{#1}%
    \def\@tempb{\nameref*{#1}}%
    \setbox0=\hbox{\@tempb}%
    \ifdim\wd0=0pt\relax\else%
      \cref@gettype{#1}{\@tempt}%
      \def\@temps{corollaryofbody}%
      \ifx\@tempt\@temps%
        ~aus~\@tempb%
      \else%
        ~\quot{\@tempb}%
      \fi%
    \fi%
}%

\def\namecref#1{%
  \def\@namecref@labelexists{0}%
  \expandafter\ifx\csname r@#1@cref\endcsname\relax%
    %%% Es gibt keinen Miktex-Label
  \else%
    \def\@namecref@labelexists{1}%
  \fi%
  \expandafter\ifx\csname r@#1\endcsname\relax%
    %%% Es gibt keinen Bakoma-Label
  \else%
    \def\@namecref@labelexists{1}%
  \fi%
  \ifnum\@namecref@labelexists=0%
    \protect\G@refundefinedtrue%
    \nfss@text{\reset@font\bfseries ??}%
    \@latex@warning{Reference `#1' on page \thepage \space undefined}%
  \else%
      \@namecref{#1}%
  \fi%
}%


\def\corollaryofref#1{\cref{#1} \quot{\nameref*{#1}}}
\newenvironment{corollaryof}[1][]{\begin{corollaryofbody}[\corollaryofref{#1}]}{\end{corollaryofbody}}

\makeatother
